Tokenisation is not in APX

In this paper, we prove that, unless P=NP, no polynomial-time algorithm can find a tokeniser whose objective is within any constant factor of the optimum, meaning that tokenisation is not in the APX complexity class. We prove this for direct and bottom-up tokenisation, under both a compression or unigram log-likelihood objectives, and for binary or larger alphabets. We further show that, even over unary alphabets, direct tokenisation is APX-hard, and thus admits no polynomial-time approximation scheme.

==> binary_direct_figures.tex <==
% =====================================================================
% fig3.tex -- binary encoding of FINITE-WORD-RANK (full-width figure,
% (a) and (b) on separate lines). Use in main.tex with  \input{fig3}
% (labels: fig:fwr, fig:fwr_enc, fig:fwr_cut). Needs only packages and
% macros main.tex already loads (enc notation: \fwrpair, \fwrencoded).
% =====================================================================
\begin{figure*}[t]
\centering
% ---------------------------------------------------------------- (a)
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}[x=1mm,y=1mm,
  cell/.style={draw,minimum height=5.2mm,minimum width=14mm,inner xsep=1pt,inner ysep=0pt,outer sep=0pt,font=\footnotesize,anchor=west},
  dots/.style={cell,minimum width=7mm},
  bit/.style={cell,minimum width=6.2mm},
  lbl/.style={font=\footnotesize},
  brc/.style={decorate,decoration={brace,amplitude=3pt,raise=1.5pt}}]
  % zoomed block enc_2(a)
  \node[lbl,anchor=east] at (17,0) {$\fwrpair{\charstring{a}}{2}={}$};
  \node[bit] (z1) at (17,0) {$\symbolone$};
  \node[bit,right=0pt of z1] (z2) {$\symbolone$};
  \node[bit,right=0pt of z2] (z3) {$\symbolzero\fwrbit_1$};
  \node[bit,right=0pt of z3] (z4) {$\symbolzero\fwrbit_2$};
  \node[bit,right=0pt of z4] (z5) {$\cdots$};
  \node[bit,right=0pt of z5] (z6) {$\symbolzero\fwrbit_{\fwrcodelength}$};
  \node[bit,right=0pt of z6] (z7) {$\symbolzero$};
  \draw[brc] (z1.north west) -- (z2.north east) node[midway,above=4.5pt,lbl] {start};
  \draw[brc] (z3.north west) -- (z7.north east) node[midway,above=4.5pt,lbl] {identifier of $(\charstring{a},2)$};
  % encoded word
  \node[lbl,anchor=east] at (17,-14) {$\fwrencoded{\charstring{ab}}={}$};
  \node[cell] (a1) at (17,-14) {$\fwrpair{\charstring{a}}{1}$};
  \node[cell,right=0pt of a1] (a2) {$\fwrpair{\charstring{a}}{2}$};
  \node[dots,right=0pt of a2] (a3) {$\cdots$};
  \node[cell,right=0pt of a3] (a4) {$\fwrpair{\charstring{a}}{\fwrrep}$};
  \node[cell,right=0pt of a4] (b1) {$\fwrpair{\charstring{b}}{1}$};
  \node[cell,right=0pt of b1] (b2) {$\fwrpair{\charstring{b}}{2}$};
  \node[dots,right=0pt of b2] (b3) {$\cdots$};
  \node[cell,right=0pt of b3] (b4) {$\fwrpair{\charstring{b}}{\fwrrep}$};
  \draw[densely dashed,gray] (z1.south west) -- (a2.north west);
  \draw[densely dashed,gray] (z7.south east) -- (a2.north east);
  \draw[brc,decoration={mirror}] (a1.south west) -- (a4.south east) node[midway,below=3.5pt,lbl,text height=2.2ex,text depth=0.4ex] {$\fwrencoded{\charstring{a}}$: $\fwrrep$ blocks};
  \draw[brc,decoration={mirror}] (b1.south west) -- (b4.south east) node[midway,below=3.5pt,lbl,text height=2.2ex,text depth=0.4ex] {$\fwrencoded{\charstring{b}}$: $\fwrrep$ blocks};
  % one token per generator
  \draw[blind_magenta,line width=1.2pt] ([yshift=-26pt]a1.south west) -- ([yshift=-26pt]b4.south east)
    node[midway,below=1pt,lbl] {token $\subwordstring{\fwrencoded{ab}}$ if $\charstring{ab}\in\generatorset$};
\end{tikzpicture}
\caption{Binary encoding of the word $\word=\charstring{ab}$.}
\label{fig:fwr_enc}
\end{subfigure}

\bigskip
% ---------------------------------------------------------------- (b)
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}[x=1mm,y=1mm,
  cell/.style={draw,minimum height=5.2mm,minimum width=14mm,inner sep=0pt,outer sep=0pt,font=\footnotesize,anchor=west},
  keep/.style={cell,fill=blind_yellow!30},
  cut/.style={cell,fill=blind_magenta!15},
  lbl/.style={font=\footnotesize},
  tok/.style={blind_magenta,line width=1.2pt},
  bnd/.style={blind_magenta,line width=1.5pt}]
  % Draws a row of blocks.  #1 = y, #2 = row name, #3 = list of style/symbol/index.
  \newcommand{\fwrBlockRow}[3]{%
    \foreach \st/\sy/\ix [count=\k] in {#3} {%
      \node[\st] (#2-\k) at ({17+14*(\k-1)},#1) {$\fwrpair{\charstring{\sy}}{\ix}$};}}
  % Boundary inside a block: ticks above and below, splitting the token line.
  \newcommand{\fwrBoundary}[1]{%
    \draw[bnd] ([yshift=2.6pt]#1.north) -- (#1.north);
    \draw[bnd] (#1.south) -- ([yshift=-4.4pt]#1.south);}
  % Token line under a span, with the word read off its j*-blocks.
  % #1/#2 = start anchor/xshift, #3/#4 = end anchor/xshift, #5 = word.
  \newcommand{\fwrTokenSpan}[5]{%
    \draw[tok] ([xshift=#2,yshift=-2.5pt]#1) -- ([xshift=#4,yshift=-2.5pt]#3)
      node[midway,below=0.5pt,lbl] {$\charstring{#5}$};}
  % row 1: ab, a single token
  \node[lbl,anchor=east] at (15,0) {$\fwrencoded{\charstring{ab}}$};
  \fwrBlockRow{0}{r}{cell/a/1,cell/a/2,keep/a/3,cell/b/1,cell/b/2,keep/b/3}
  \fwrTokenSpan{r-1.south west}{1pt}{r-6.south east}{-1pt}{ab}
  % row 2: bab, a boundary inside enc_1(a)
  \node[lbl,anchor=east] at (15,-12.5) {$\fwrencoded{\charstring{bab}}$};
  \fwrBlockRow{-12.5}{s}{cell/b/1,cell/b/2,keep/b/3,cut/a/1,cell/a/2,keep/a/3,cell/b/1,cell/b/2,keep/b/3}
  \fwrBoundary{s-4}
  \fwrTokenSpan{s-1.south west}{1pt}{s-4.south}{-2pt}{b}
  \fwrTokenSpan{s-4.south}{2pt}{s-9.south east}{-1pt}{ab}
  % row 3: bb, a boundary inside the second enc_2(b)
  \node[lbl,anchor=east] at (15,-25) {$\fwrencoded{\charstring{bb}}$};
  \fwrBlockRow{-25}{t}{cell/b/1,cell/b/2,keep/b/3,cell/b/1,cut/b/2,keep/b/3}
  \fwrBoundary{t-5}
  \fwrTokenSpan{t-1.south west}{1pt}{t-5.south}{-2pt}{b}
  \fwrTokenSpan{t-5.south}{2pt}{t-6.south east}{-1pt}{b}
  % legend
  \node[keep,minimum width=4.5mm,minimum height=3.4mm] (k) at (17,-37) {};
  \node[lbl,anchor=west] at (k.east) {never cut ($j^\star{=}3$)};
  \node[cut,minimum width=4.5mm,minimum height=3.4mm] (c) at (51,-37) {};
  \draw[bnd] ([yshift=1.8pt]c.north) -- (c.north) (c.south) -- ([yshift=-1.8pt]c.south);
  \node[lbl,anchor=west] at (c.east) {cut};
  \draw[tok] (70,-37) -- (75,-37);
  \node[lbl,anchor=west] at (75,-37) {token};
\end{tikzpicture}
\caption{Tokenising $\wordset=\{\charstring{ab},\charstring{bab},\charstring{bb}\}$, with $\fwrrep=3$.}
\label{fig:fwr_cut}
\end{subfigure}
\caption{
(a)~Each symbol becomes $\fwrrep$ blocks $\fwrpair{\character}{j}$, each a start marker $\symbolone\symbolone$ followed by an identifier of $(\character,j)$.
(b)~Each boundary cuts at most one block, so fewer than $\fwrrep$ boundaries leave some index $j^\star$ uncut; the $j^\star$-blocks of each token spell a word, and these words generate $\wordset$.
}
\label{fig:fwr}
\end{figure*}

==> blowup_figure.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    blowclone/.style={circle,draw,fill=white,minimum size=3mm,inner sep=0pt},
    blowcluster/.style={draw=black!35,fill=black!4,rounded corners=2.6mm,line width=0.4pt},
  ]
  % one colour per edge of G; the edges it becomes in G_3 share it
  \colorlet{blowab}{blind_blue}
  \colorlet{blowbc}{blind_magenta}
  \colorlet{blowca}{blind_orange}

  % --- the graph G ---
  \node[buvtx] (a) at (90:0.95)  {$a$};
  \node[buvtx] (b) at (210:0.95) {$b$};
  \node[buvtx] (c) at (330:0.95) {$c$};
  \draw[blowab,thick] (a) -- (b);
  \draw[blowbc,thick] (b) -- (c);
  \draw[blowca,thick] (c) -- (a);
  \node[font=\small] at (0,-1.7) {$\srcgraph$};

  \draw[-latex,thick] (1.55,0.1) -- node[above,font=\small] {$t=3$} (2.75,0.1);

  % --- its 3-blow-up G_3 ---
  \begin{scope}[xshift=5.15cm]
    \def\R{1.7}  % distance of the clusters from the centre
    \def\d{0.42} % spacing of clones within a cluster
    \foreach \v/\ang in {a/90, b/210, c/330} {
      \begin{scope}[shift={(\ang:\R)}, rotate=\ang+90]
        \draw[blowcluster] (-0.72,-0.27) rectangle (0.72,0.27);
        \coordinate (\v1) at (-\d,0);
        \coordinate (\v2) at (0,0);
        \coordinate (\v3) at (\d,0);
      \end{scope}
      \node[font=\small] at ({\ang}:{\R+0.6}) {$\v$};
    }
    \foreach \u/\w/\col in {a/b/blowab, b/c/blowbc, c/a/blowca} {
      \foreach \i in {1,2,3} {
        \foreach \j in {1,2,3} {
          \draw[\col, line width=0.45pt] (\u\i) -- (\w\j);
        }
      }
    }
    \foreach \v in {a,b,c} {
      \foreach \k in {1,2,3} {
        \node[blowclone] at (\v\k) {};
      }
    }
    \node[font=\small] at (0,-1.7) {$\srcgraph_3$};
  \end{scope}
\end{tikzpicture}
\caption{
The $3$-blow-up of a triangle (\cref{def:blowup}).
Each edge becomes a complete bipartite graph between two clusters, drawn in the edge's colour.
}
\label{fig:blowup}
\end{figure}
